AU-AIR: A Multi-modal Unmanned Aerial Vehicle Dataset for Low Altitude Traffic Surveillance

Unmanned aerial vehicles (UAVs) with mounted cameras have the advantage of capturing aerial (bird-view) images. The availability of aerial visual data and the recent advances in object detection algorithms led the computer vision community to focus on object detection tasks on aerial images. As a result of this, several aerial datasets have been introduced, including visual data with object annotations. UAVs are used solely as flying-cameras in these datasets, discarding different data types regarding the flight (e.g., time, location, internal sensors). In this work, we propose a multi-purpose aerial dataset (AU-AIR) that has multi-modal sensor data (i.e., visual, time, location, altitude, IMU, velocity) collected in real-world outdoor environments. The AU-AIR dataset includes meta-data for extracted frames (i.e., bounding box annotations for traffic-related object category) from recorded RGB videos. Moreover, we emphasize the differences between natural and aerial images in the context of object detection task. For this end, we train and test mobile object detectors (including YOLOv3-Tiny and MobileNetv2-SSDLite) on the AU-AIR dataset, which are applicable for real-time object detection using on-board computers with UAVs. Since our dataset has diversity in recorded data types, it contributes to filling the gap between computer vision and robotics. The dataset is available at https://bozcani.github.io/auairdataset.

==> temp.tex <==
\subsection{Network Training Performance}

We calculate a mean squared error on difference between the input and reconstructed data and observed how it changes during training:
\begin{equation}
E_{train} = \frac{1}{N}\sum_{i}^N {(\mathbf{x}_i - \mathbf{\hat{x}}_i)^2},
\label{train_error_equation}
\end{equation}
where $\mathbf{x}_i$ is the $i^{th}$ input grid vector in the dataset which has $N$ number of samples, and $\mathbf{\hat{x}}_i$ is corresponding reconstructed grid vector for $x_i$.

We look training and validation loss separately for baselines. We observe that without copy-crop links (CVAE and VAE) have higher reconstruction error regardless of feeding gps inputs. Moreover, feeding gps data as input to the networks (UAV-AdNet) causes lower reconstructed error compared to the network (UAV-AdNet-wo-gps).
\begin{figure}[!hbt] 
\centerline{
\includegraphics[width=0.49\textwidth]{figures/error_vs_epoch.pdf}
}
\caption{Reconstruction error vs epochs plot during training. Solid and dashed lines indicates training and validation errors respectively. Black colored lines belongs to network architecture with gps input and copy-crop link for the grid inputs. Red colored lines belong to the network architecture without gps input and with copy-crop link for the grid inputs. }
\end{figure}





%Table
\begin{table}[hbt!]
\caption{Comparison with existing studies on Scene Modeling for robots. $V^{3d}$:3D points and image from RGBD sensors; $V^{2d}$: RGB image from on board camera; A: Audial from microphone; H: Haptic from sensors; O: Ontological knowledge entity for any type of modality; GPS: GPS data ; UGV: Unmanned Ground Vehicle; UAV: Unmanned Aerial Vehicle; n/a: Robot platform is not mentioned in original work. 
\label{tbl:comparison}}
\begin{center}
\footnotesize
\begin{tabular}{c|cccc}\hline
Study & Main Method & Data & Robot & Task \\  
 &  & Modality & Platform & Env. \\  \hline \hline


\cite{CelikkanatConceptWeb2014}  & MRF & V^{3d}, A, H & humanoid robot & indoor \\
\cite{anand2013contextually}  & MRF & V^{3d} & UGV & indoor \\
\cite{lin2013holistic} & MRF & V^{3d} & n/a & indoor \\

\cite{li2017context} & BN & O & underwater robot & underwater \\

\cite{joho2013nonparametric} & DB process & V^{3d} & service robot & indoor \\

\cite{mastrogiovanni2011robots} & PL & O & UGV & indoor \\

\cite{hwang2006ontology} & Ontology & O & n/a & indoor \\

\cite{saxena2014robobrain, tenorth2009knowrob} & Ontology & O & service robot & indoor \\

\cite{bozcan2019cosmo, bozcan2018missing} & BM & V^{3d} & humanoid robot& indoor \\

\hline
our & H, DNN & V^{2d}, GPS & UAV & outdoor  \\
method &&  &  &   \\
\hline

\end{tabular}
\end{center}

\end{table}








Firstly, we remove gps input layer from UAV-AdNet and train and test it with input grid vectors only. We call this model as UAV-AdNet-wo-gps. Secondly, we remove copy-crop links for grid input layer from UAV-AdNet and keep gps input layer. This network has type of conditional variational autoencoder (CVAE) where the model is conditioned on gps data. Lastly, we use regular Variation Autoencoder (VAE) by removing both copy-crop links for input layer and gps inputs. Baseline summaries can be shown in Table \ref{tbl:baselines} .

 \begin{table}[hbt]
\caption{Baseline architectures compared to proposed network UAV-AdNet. \label{tbl:baselines}}
\centering
\begin{tabular}{|ccc|}\hline                                                                 
Network  & Gps inputs  & Copy-crop links \\ \hline \hline
UAV-AdNet &  yes    &  yes \\ \hline
UAV-AdNet-wo-gps &  yes    &  no \\ \hline
CVAE &  yes    &  no \\ \hline
VAE &  no    &  no \\ \hline
\end{tabular}
\end{table}
 







\subsection{Anomaly Detection Task}
%Our model can find anomalies (i.e. suspicious existence of objects) in given environment. For testing, we prepared test data and split it into three categories that each has different anomaly scenarios. The first category includes anomalies which violates security rules of DeepTech Experimental Hub (such as a person at the forbidden area -back side of the building-, a car in front of exits etc.). The second category includes anomalies which are not parts of DeepTech Experimental Hub rules  but belong to public rules (such as a car at the bike road, person on the road). The third category includes anomalies which are not part of neither private nor public rules. Therefore, it is difficult to detect these cases since they are implicit and require long-term observation of the environment. Rare existence of objects belong to this category (such as human at the right side of the building, trucks at the parking area of the building etc.)

Our model can find anomalies (i.e. suspicious existence of objects) in given environment. For testing, we split test data into three categories that each has different anomaly scenarios. The first anomaly category (Scenario 1) includes anomalies which breaks specific rules related to interested surveillance area (e.g. a person at the forbidden zone). The second anomaly category (Scenario 2) consists of anomalies which breaks public rules and they are not directly related to private rules (e.g. a car at the bike road). The third anomaly category (Scenario 3) includes anomalies which do not break neither private or public rules. Although these cases do not break any rules, they may raise suspicion due to rare occurrence (e.g. a truck at car parking area). Qualitative examples are given in Figure \ref{fig:scenerios}

\begin{figure}[hbt] 
\centerline{
\includegraphics[width=0.49\textwidth]{figures/scenarios_compressed.pdf}
}
\caption{Example images for different anomaly scenarios. Red and blue rectangles show anomaly and normal objects respectively. The left image indicates a case breaking of private rules of the area (Scenario 1). Humans are not allowed to enter back side of the building. The middle image shows a case breaking of public rule (Scenario 2). Bikes are not allowed to use vehicle roads. Right image shows an example of rare observation of objects which may arise suspicions. Bikes are usually parked at the bike parking area instead of car park of the building.\label{fig:scenerios}}
\end{figure}



%area private rules (i.e. private rules of DeepTech Experimental Hub) such as a person at the forbidden area (e.g. back side of the building).

For testing Scenario 1, we choose test samples which include cases breaking private rules. Moreover, we create syntactic scene representations by adding objects randomly into ground truth input grid vectors to increase the size of test set. Objects are chosen and put in order to create scene representations which include private rules breaking cases. Same method is applied to create synthetic scene representations for Scenario 2 and 3.


%Next, we evaluate our model with Scenario 2. For this end, we use real and synthetic samples as well. Lastly, we use only real samples to test Scenario 3 since the model is supposed to find anomalies for undefined rules. Therefore, creating syntactic samples for Scenario 3 does not make sense since this type of anomalies may not be defined and recognized by human. %For all scenarios, we define accuracy as the percentage of objects correctly estimated with respect to the labeled objects in the test dataset.

For evaluating the performance of the methods, we use precision, recall and F1-score which are defined as follows:
%
\begin{eqnarray}
\textrm{Precision} & = & \frac{\textrm{TP}}{\textrm{TP}+\textrm{FP}},\\
\textrm{Recall} & = & \frac{\textrm{TP}}{\textrm{TP}+\textrm{FN}},\\
\textrm{F1-score} & = & 2\cdot \frac{\textrm{Precision}\cdot \textrm{Recall}}{\textrm{Precision} + \textrm{Recall}},
\end{eqnarray}
%
{\noindent}where TP, FP and FN stand for the number of true positives, false positives and false negatives, respectively. For anomaly detection task, we define TP as the number of grid cells that have value $0$ in reconstructed data correctly according to the ground truth sample; FP as the number of grid cells that the model set value $1$ but should have been $0$ according to the ground truth; TN as the number of grid cells that are set to $0$ correctly according to ground truth, and FN as the number of objects that the model is set to $0$, yet should have been $1$ according to the ground truth. We can formally define these as follows: 
%
\begin{eqnarray}
TP & = & \left\vert \{x: x\in {G^1} \land x\in {M^1}  \} \right\vert , \label{eqn:task2hypothesiseqns} \\
TN & = & \left\vert \{x: x\in {G^0} \land x\in {M^0}  \} \right\vert , \nonumber \\
FP & = & \left\vert \{x: x\in {G^0} \land x\in {M^1}  \} \right\vert , \nonumber \\
FN & = & \left\vert \{x: x\in {G^1} \land x\in {M^0}  \} \right\vert \nonumber ,
\end{eqnarray}
%
{\noindent}where $x$ is an instance of a reconstructed grid vector that indicates existence of an object; ${G^1}$ and ${G^0}$ are the sets of grid cells which have value $1$ and $0$ respectively in the ground truth sample; and ${M^1}$ and ${M^0}$ are the sets of grid cells which have value $1$ and $0$ respectively at the end of the model's reconstruction.


As shown in Table \ref{tbl:results}, proposed method performs better than baselines for all scenarios. For Scenerio 1, 

% \begin{table}[hbt]
%\caption{Baseline architectures compared to proposed network UAV-AdNet. %\label{tbl:results}}
%centering
%\begin{tabular}{|cccc|}\hline                                                                 
%Network  & Scenerio 1  & Scenerio 2 & Scenerio 3 \\ \hline \hline
%UAV-AdNet &  \textbf{98.2\%}    &  \textbf{92.6\%} &  \textbf{81.7\%}  \\ \hline
%UAV-AdNet-wo-gps & 86.8 \% & 81.0\% & 75.3\% \\ \hline
%CVAE & 69.2\%    & 61.3\% & 57.2\%\\ \hline
%VAE &  67.1\%    & 61.3\% & 56.7\%\\ \hline
%\end{tabular}
%\end{table}

\begin{table}[hbt]
\caption{Scenerio 1 performances. \label{tbl:whatismissing}}
\centering
\footnotesize
\begin{tabular}{|l|ccc|}\hline                                                                 
&\textbf{Precision}  & \textbf{Recall}  & \textbf{F1-score}  \\ \hline \hline
UAV-AdNet & \textbf{0.9816}	& \textbf{1.0}   & \textbf{0.9907}   \\ 
UAV-AdNet-wo-gps & 0.9427 & 0.9984  &  0.9697  \\ 
CVAE & 0.1963 & 0.5165  &  0.2845   \\ 
VAE  & 0.1920	 &  0.4102   &  0.2616 \\ \hline
  
\end{tabular}
\end{table}


\begin{table}[hbt]
\caption{Scenerio 2 performances. \label{tbl:whatismissing}}
\centering
\footnotesize
\begin{tabular}{|l|ccc|}\hline                                                                 
&\textbf{Precision}  & \textbf{Recall}  & \textbf{F1-score}  \\ \hline \hline
UAV-AdNet & \textbf{0.9724}	& \textbf{0.9899}   & \textbf{0.9811}   \\ 
UAV-AdNet-wo-gps & 0.9621 & 0.99  &  0.9759  \\ 
cVAE & 0.1982 & 0.3955  &  0.2641   \\ 
VAE  & 0.1979	 &  0.3992   &  0.2646 \\ \hline
  
\end{tabular}
\end{table}

\begin{table}[hbt]
\caption{Scenerio 3 performances. \label{tbl:whatismissing}}
\centering
\footnotesize
\begin{tabular}{|l|ccc|}\hline                                                                 
&\textbf{Precision}  & \textbf{Recall}  & \textbf{F1-score}  \\ \hline \hline
UAV-AdNet & \textbf{0.9630}	& \textbf{0.9939}   & \textbf{0.9782}   \\ 
UAV-AdNet-wo-gps & 0.9517 & 0.9939  &  0.9723  \\ 
cVAE & 0.1958 & 0.5158  &  0.2839   \\ 
VAE  & 0.1990	 &  0.4113   &  0.2682 \\ \hline
  
\end{tabular}
\end{table}


\begin{table}[hbt]
\caption{Anomaly detection accuracy. \label{tbl:whatismissing}}
\centering
\footnotesize
\begin{tabular}{|l|ccc|}\hline                                                                 
&\textbf{Scenario 1}  & \textbf{Scenario 2}  & \textbf{Scenario 3}  \\ \hline \hline
UAV-AdNet & \textbf{0.9214}	& \textbf{0.8614}   & \textbf{0.8255}   \\ 
UAV-AdNet-wo-gps & 0.8778 & 0.7912  &  0.7778  \\ 
cVAE & 0.6212 & 0.4413  &  0.4433   \\ 
VAE  & 0.6198	 &  0.4165   &  0.42 \\ \hline
  
\end{tabular}
\end{table}




%abstract
In this paper, we present a variant of deep neural networks (UAV-AdNet) which is trained in unsupervised manner for autonomous anomaly detection using UAVs. For this end, firstly, we propose grid-wise environment representation of bird-view images captured by UAVs. Secondly, we propose ..., a variant of VAE, that learns joint distribution of grid-wise scene representation of aerial images and corresponding gps labels recorded by the UAVs. We evaluate our model against several baselines on a aerial surveillance dataset, and show that it performs better in anomaly detection task.


\subsection{The Properties of the Dataset}
AU-AIR dataset consists of ?(~16) video clips (~4 hours long in total) with nearly 70,000 frames. The videos are captured at Skejby in Aarhus city with low altitude flights (max. 30 meter). To increase the challenge depending the altitude, the drone has flown at 10, 20 and 30 meters during recordings \IB{give stats}. Moreover, camera angle has been changed from 90 degree (complete bird-view images) to 45 degree. The perspective in aerial images increases from 45 degree to 90 degree that change the view of an image.

The videos has been recorded in different times. The time changes the layout and the density of object instances in an environment \IB{give stats}. Moreover, in our dataset, the illumination in the images also varies according the day time.

Some of the videos has been recorded while the drone is stabilized in the air but turning around itself. It keeps the location coordinates constant but changes the IMU data (i.e., roll, pitch, yaw angles) and image views. There are also video records which are captured while the drone has horizontal velocity (i.e., X and Y axis) and vertical axis (i.e., Z axis) in the air \IB{give stats}.





\section{INTRODUCTION}
By the advance in low weight sensors, UAVs can capture a wide range of visual data types (e.g., RGB images and videos, thermal images, multi-spectral images) according to the specific application. In addition to the visual data, they can record the other sensory data using internal sensors (e.g., yaw, pitch, roll form the IMU sensor, the location coordinates from a GPS sensor, the altitude from a barometer sensor) during their flight. Although some of sensory data are discarded for an application, some might help to increase the application performance.

Object detection in aerial images is one of the wildly studied process in UAV applications. The recent on-board computers (e.g., NVIDIA Jetson TX2, Intel Nuke i7) allows camera mounted UAVs to conduct real time object detection in aerial images. 

\begin{figure}[hbt]
    \centering
    \includegraphics[width=0.49\textwidth]{figures/intro.pdf}
    \caption{Introduction [Best viewed in color]}
    \label{fig:intro}
\end{figure}

Deep learning has brought the state-of-the-art results for the object detection task. The variants of deep convolutional neural networks are the fundamental methods that achieve the breakthrough results. Although there are a wild number of datasets for object detection, the vast majority of them consists of natural images or videos captured by humans using handheld cameras. However, the images captured by UAVs have bird-view perspective which makes object appears shorthanded and small. The significant difference between the view of natural images and aerial images causes that the state-of-the-art object detectors which are studied for the natural images works poorly for aerial images. %Therefore, several datasets have been proposed for object detection in aerial images captured by UAVs. 


By the recent advance in object detection performances using deep learning methods, the computation power and large datasets, several datasets that are dedicated to object detection in aerial images have been introduced. Since they have been proposed for computer vision tasks (mainly object detection and tracking), other sensory data recorded by UAVs are discarded. Although these datasets fill the gap between drones and computer vision, to the best of our knowledge, there is no real world drone dataset which includes multi-modal data recorded during flights.

As an example of a robotic platform, self-driving (autonomous) cars have a variety of sensors similar to the UAVs. In recent years, a variety of self-driving car datasets that includes multi-modal data (e.g., RGB images, depth images, IMU, GPS, odometry) has been introduced to meet computer vision with robotics. Our dataset targets the same aim for UAVs.

In this paper, we present a multi-modal UAV dataset (The AU-AIR dataset) in order to push forward the development of computer vision and robotic algorithms targeted to autonomous aerial surveillance using a UAV. The AU-AIR dataset consists of video streams for the traffic surveillance that are captured in Aarhus, Denmark. The videos mainly records a circular intersection of Skejby Nordlandsvej and P.O Pedersensvej and the roads itself. The dataset includes aerial videos, GPS coordinates and the altitude of the drone, IMU data, and the velocity. The videos are recorded in different camera angles from 45 degree to 90 degree (i.e., complete bird-view images that the camera is perpendicular to the Earth). Eight object categories which are highly related to aerial surveillance (i.e., person, car, van, truck, motorbike, bike, bus, trailer) are annotated with bounding boxes in video frames.

In our experiments, we analyze the main challenges of the object detection in aerial images compared to the natural images. Since, we consider real-time object detection task with drones, we use light-weight object detectors (YOLO-tiny and MobileNetV2-SSD Lite) that can make inferences on board computers with a high frame rate.

%In this paper, we present a UAV dataset including multi-modal sensor data including videos, GPS location, the altitude, the velocity, IMU data and the flight time.


%video streams with annotated ground-truth bounding boxes for predefined object labels. Moreover, we provide GPS locations corresponding image frames, and current time, IMU data, the altitude and battery level of the UAV. The benchmark dataset consists of ? video clips which are split into ? frames in total. We have captured video clips around Aarhus University DeepTech Experimental Hub in Aarhus, Denmark during the aerial surveillance of the building. We have labelled 8 types of object in total for all frames: person, car, truck, van, bike, motorbike, trailer, tractor. These objects are selected as the interest of surveillance. Video clips are saved in low altitude UAV flights (max. 30 meters) and in different locations and orientations of the UAV. The current recording time of the video clips are also added to the dataset with the data regarding UAV battery level.




%By the advance in low weight sensors and on-board computers, unmanned aerial vehicles (UAVs) have been deployed to various applications in different fields such as agriculture, surveillance, and inspection. For these applications, UAVs record a wide range of data such as images, videos, current time, GPS locations, IMU measurements during the flight. For each operation, some of the data might be relevant, but others do not. Therefore, irrelevant sensor data are discarded for the given operation.

%Among the applications which UAVs are deployed, most of them are related to computer vision such as object detection, object tracking, activity recognition thanks to the great progress in deep learning based computer vision algorithms. Therefore, they rely on only images or videos and discard other flight data.

%The focusing on visual data emerges variety of datasets which consist of aerial images captured by UAVs. These UAVs-generated visual datasets are applicable for several tasks including activity recognition, object detection or object tracking without using different data modalities. Therefore, although there are several datasets and benchmarks for UAV vision datasets, to the best of our knowledge, there is no public dataset including multi-modal data captured in real environment. Our motivation is to fill this gap providing multi-modal UAV dataset that can be used for different purposes.



%Since real time understanding of visual data might be crucial for UAV-deployed applications, we have trained and evaluated tiny state-of-the-art object detectors (including tiny yolo and mobilenet-ssd) that can make inference on board computers with higher frame rate. We have ignored cumbersome state-of-the-art object detectors such as FasterRCNN, RetinaNet, YOLOV3 since they are not feasible for real time inferences using on board computers. We compare these two baseline networks in terms of the accuracy and the inference time in different on-board computers which are extensively used in robotics.


%Moreover, the operational difficulties of gathering data with UAVs causes to the presenting of artificial datasets as well.

% Low weight sensorler ve ucus kabileyetleri sayesinde

